LLM Unlearning Reveals a Stronger-Than-Expected Coreset Effect in Current Benchmarks

Large language model unlearning has become a critical challenge in ensuring safety and controlled model behavior by removing undesired data-model influences from the pretrained model while preserving general utility. Significant recent efforts have been dedicated to developing LLM unlearning benchmarks such as WMDP (Weapons of Mass Destruction Proxy) and MUSE (Machine Unlearning Six-way Evaluation), facilitating standardized unlearning performance assessment and method comparison. Despite their usefulness, we uncover for the first time a novel coreset effect within these benchmarks. Specifically, we find that LLM unlearning achieved with the original (full) forget set can be effectively maintained using a significantly smaller subset (functioning as a "coreset"), e.g., as little as 5% of the forget set, even when selected at random. This suggests that LLM unlearning in these benchmarks can be performed surprisingly easily, even in an extremely low-data regime. We demonstrate that this coreset effect remains strong, regardless of the LLM unlearning method used, such as NPO (Negative Preference Optimization) and RMU (Representation Misdirection Unlearning), the popular ones in these benchmarks. The surprisingly strong coreset effect is also robust across various data selection methods, ranging from random selection to more sophisticated heuristic approaches. We explain the coreset effect in LLM unlearning through a keyword-based perspective, showing that keywords extracted from the forget set alone contribute significantly to unlearning effectiveness and indicating that current unlearning is driven by a compact set of high-impact tokens rather than the entire dataset. We further justify the faithfulness of coreset-unlearned models along additional dimensions, such as mode connectivity and robustness to jailbreaking attacks. Codes are available at https://github.com/OPTML-Group/MU-Coreset.

==> Fig_texs/fig1.tex <==
\begin{wrapfigure}{r}{105mm}
\vspace*{-5mm}
\centering
\includegraphics[width=.75\textwidth]{Figs/Fig1.pdf}\\
\vspace{-1mm}
\begin{tabular}{cc}
\hspace*{20mm} \scriptsize{(a) Trajectory of UE vs epochs} 
& \hspace*{10mm}
\scriptsize{(b) Model utility preservation} 
\end{tabular}
\vspace*{-7mm}
\caption{\footnotesize{Unlearning effectiveness (\textbf{a}) using RMU gets better as epochs increase while utility (\textbf{b}) is maintained (where box plots represent the distribution of UT across epochs) for different values of $\mathrm{p} = 0.1, 0.05, 0.01$ in WMDP-Bio.
}}
  \label{fig: fig1}
  \vspace*{-6mm}
\end{wrapfigure}

==> Fig_texs/fig2_CLE.tex <==
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=\linewidth]{Fig_texs/CLE_Fig2_1row.pdf}
%     \caption{\footnotesize{Randomly selected subsets from WMDP from the full forget set has good unlearning performance.}}
%     \label{fig: cle}
% \end{figure}
\begin{wrapfigure}{r}{90mm}
% \vspace*{-5mm}
\centerline{
\includegraphics[width=.65\textwidth,height=!]{Figs/CLE_Fig2.png}}
% \vspace*{-3mm}
\caption{\footnotesize{Randomly selected subsets from WMDP from the full forget set has good unlearning performance.
}}
  \label{fig: fig1}
  % \vspace*{-6mm}
\end{wrapfigure}

==> Tables/musebooks.tex <==
\begin{table}[htb]
\begin{center}
% \vspace{-2mm}
\caption{\small{Coreset-based unlearning performance (UE and UT, consistent with Fig. 2) using RMU and NPO on MUSE evaluated using LLaMA2-7B on News and ICLM-7B on Books. The table is presented in the same format as \reftab{tab: wmdp-bio}. Here `Retrain' refers to a model finetuned only on MUSE excluding the forget set.
} 
}
\vspace*{2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|ccc|c|ccc|c}
\toprule[1pt]
\midrule

\multicolumn{1}{c|}{\multirow{4.5}{*}{
\begin{tabular}{c}
   \textbf{Coreset} \\
     \textbf{Ratio}
\end{tabular}
}} 
&\multicolumn{1}{c|}{\multirow{4.5}{*}{
\begin{tabular}{c}
     \textbf{Unlearning} \\
     \textbf{Method}
\end{tabular}
}} 
& \multicolumn{4}{c|}{\textbf{RMU}} 
&  \multicolumn{4}{c}{\textbf{NPO}} \\
\cmidrule{3-10}
&& \multicolumn{3}{c|}{\textbf{UE}} 
& \multicolumn{1}{c|}{\textbf{UT}} 
& \multicolumn{3}{c|}{\textbf{UE}} 
& \multicolumn{1}{c}{\textbf{UT}} \\
\cmidrule{3-10}
&& \begin{tabular}{c}
   \textbf{VerbMem} \\
      ($\downarrow$) 
\end{tabular}
& \begin{tabular}{c}
   \textbf{KnowMem} \\
      ($\downarrow$) 
\end{tabular}
& \begin{tabular}{c}
   \textbf{PrivLeak} \\
      ($\rightarrow$ 0)
\end{tabular} 
& \begin{tabular}{c}
   \textbf{KnowMem} \\
      ($\uparrow$) 
\end{tabular}
& \begin{tabular}{c}
   \textbf{VerbMem} \\
      ($\downarrow$) 
\end{tabular}
& \begin{tabular}{c}
   \textbf{KnowMem} \\
      ($\downarrow$) 
\end{tabular}
& \begin{tabular}{c}
   \textbf{PrivLeak} \\
      ($\rightarrow$ 0)
\end{tabular} 
& \begin{tabular}{c}
   \textbf{KnowMem} \\
      ($\uparrow$) 
\end{tabular}
\\ 
\midrule
\multicolumn{10}{c}{\textbf{MUSE-Books}}\\
\midrule
0\% & No unlearning &
99.56  & 58.32  & -56.32   & 67.01
&
99.56  & 58.32  & -56.32   & 67.01
 \\
\midrule
0\% & Retrain &
14.30 & 28.90 & 0.00   & 74.50 
&
14.30 & 28.90 & 0.00   & 74.50 
 \\
\midrule
100\% & Full forget Set
& 5.38 %$_{\pm{0.17}}$ 
& 18.72 %$_{\pm{13.49}}$ 
&  -16.98 %$_{\pm{10.41}}$ 
& 40.34 %$ %_{\pm{24.50}}$  
& 0.00 %$ %_{\pm{0.00}}$ 
& 0.00 %$_{\pm{0.00}}$ 
&  -31.02 %$_{\pm{1.04}}$ 
& 31.33 %$_{\pm{3.67}}$ 
\\
\midrule
\multirow{4}{*}{
\begin{tabular}{c}
   10\% 
\end{tabular}
}
& \random{}
& 4.34$_{\pm{1.40}}$ 
& 23.86$_{\pm{10.79}}$ 
&  -12.79$_{\pm{4.86}}$ 
& 56.67$_{\pm{7.29}}$  
& 0.00$_{\pm{0.00}}$ 
& 0.00$_{\pm{0.00}}$ 
&  -27.09$_{\pm{2.22}}$ 
& 29.12$_{\pm{3.36}}$\\
&\grand{}
& 4.96
& 21.69
& 5.07
& 57.11
& 0.00
& 0.00
&  -25.28
& 37.54\\
& \moderate{}
& 5.72
& 9.02
& -19.84
& 33.44
& 0.00
& 0.00
& -28.42
& 36.55\\
%%%  Mink for NPO 0.5
& \mink{}
& 7.53
& 20.12
& -29.17
& 56.43
& 0.00
& 0.00
& -0.24
& 33.21 \\
\midrule
\multirow{4}{*}{
\begin{tabular}{c}
   5\% 
\end{tabular}
}
%%%  random for RMU 0.5
& \random{}
& 4.01$_{\pm{1.58}}$ 
& 19.37$_{\pm{6.75}}$ 
&  -18.61$_{\pm{1.88}}$ 
& 54.62$_{\pm{5.54}}$  

%%%  random for NPO 0.5
& 0.00$_{\pm{0.00}}$ 
& 3.48$_{\pm{0.56}}$ 
&  -8.97$_{\pm{8.03}}$ 
& 36.19$_{\pm{1.35}}$\\
&\grand{}
%%%  grand for RMU 0.5
& 5.69
& 28.00
& -37.66
& 59.21

%%%  grand for NPO 0.5
& 0.00
& 3.77
&  -15.71
& 40.15 \\  
& \moderate{}
%%%  Moderate for RMU 0.5
& 4.75
& 7.08
& -18.02
& 33.92

%%%  Moderate for NPO 0.5
& 0.00
& 3.35
&  -5.63
& 36.93\\ 
%%%  Mink for RMU 0.5
& \mink{}
& 4.20
& 37.48
& -0.12
& 67.76

%%%  Mink for NPO RMU 0.5
& 0.00
&  4.33
& -32.90
& 39.18\\

%%% MUSE NEWS
\midrule
\multicolumn{10}{c}{\textbf{MUSE-News}}\\
\midrule
0\% & No unlearning &
58.29  & 62.93  & -98.71    & 54.31
&
58.29  & 62.93  & -98.71    & 54.31
 \\
\midrule
0\% & Retrain &
20.75 & 33.32 & 0.00    & 53.79
&
20.75 & 33.32 & 0.00    & 53.79
\\
 \midrule
100\% & Full forget set
%%%  Random for RMU 1
& 21.00 
& 54.68 
&  1.80 
& 44.75 

%%%  Random for NPO 1
& 0.00 
& 47.96 
&  107.40 
& 37.86 
\\
\midrule
\multirow{4}{*}{
\begin{tabular}{c}
   10\% 
\end{tabular}
}
& \random{}
%%%  Random for RMU 0.1
& 29.97$_{\pm{2.50}}$ 
& 18.85$_{\pm{21.99}}$ 
&  -38.87$_{\pm{2.78}}$ 
& 50.23$_{\pm{1.67}}$  

%%%  Random for NPO 0.1
& 20.54$_{\pm{1.71}}$ 
& 42.30$_{\pm{1.26}}$ 
&  -99.58$_{\pm{0.14}}$ 
& 38.54$_{\pm{0.61}}$\\
&\grand{}
& 28.85
& 40.50
& -45.84
& 49.50
& 21.35
& 41.97
& -99.71
& 38.59
\\
& \moderate{}
& 32.62
& 38.40
& -36.44
& 52.77
& 19.26
& 42.46
& -99.78
& 37.99
\\
%%%  Mink for NPO 0.5
& \mink{}
& 31.67
& 2.02
& -15.95
& 50.14
& 23.59
& 43.85
& -98.14
& 40.66 \\
\midrule
\multirow{4}{*}{
\begin{tabular}{c}
   5\% 
\end{tabular}
}
%%%  random for RMU 0.5
& \random{}
& 20.15$_{\pm{7.50}}$ 
& 12.95$_{\pm{17.17}}$ 
&  -16.42$_{\pm{18.70}}$ 
& 40.93$_{\pm{4.32}}$  


%%%  random for NPO 0.5
& 7.36$_{\pm{0.79}}$ 
& 34.28$_{\pm{1.92}}$ 
&  -76.38$_{\pm{7.46}}$ 
& 32.75$_{\pm{1.75}}$ \\
&\grand{}
%%%  grand for RMU 0.5
& 24.15
& 50.26
& -33.27
& 47.11

%%%  grand for NPO 0.5
& 3.51
& 32.71
& -1.85
& 31.65 \\  
& \moderate{}
%%%  Moderate for RMU 0.5
& 19.37
& 52.21
& -8.53
& 47.00

%%%  Moderate for NPO 0.5
& 3.19
& 38.24
& 16.50
& 35.57 \\ 
%%%  Mink for RMU 0.5
& \mink{}
& 28.83
& 49.21
& -33.74
& 43.94

%%%  Mink for NPO RMU 0.5
& 3.40
&  36.45
& 73.07
& 31.21\\

\midrule
\bottomrule
\end{tabular}
}
\label{tab: muse}
% \vspace*{-2mm}
\end{center}
\end{table}

==> secs/abstract.tex <==

We uncover a novel Coreset Effect in current LLM unlearning benchmarks, 
% where we show that unlearning performance using the original forget set is achievable using very small subsets of the forget set, for e.g. as little as  5\% of the forget set.
we show that the unlearning performance achieved with the original forget set can be maintained using significantly smaller subsets, such as just 5\% of the forget set.
% where we can achieve good unlearning performance with very small subsets of the forget dataset, for e.g. as little as  5\% of the original forget set.
Surprisingly, this coreset effect can be even be achieved through randomly chosen subsets of the forget set and is consistent across different state-of-the-art unlearning methods (e.g., NPO and RMU) in standard benchmarks like WMDP and MUSE. 
% We demonstrate nlearned models using smaller subsets of forget set can even sometimes demonstrate better performance. Additionally, 
Along with random selection, we demonstrate this effect using various heuristics-based coreset selection methods, which have marginal advantages over random selection. 
We explain this phenomenon through a keyword perspective by extracting keywords from the forget set and unlearning using solely such keywords. Models unlearned with keywords explain a significant portion of unlearning performance which is achieved using the forget set. 
Additionally, we show the reliability of this Coreset Effect through various perspectives such as mode connectivity, emergent utility metrics and adversarial robustness against jailbreaking attacks. Coreset-unlearned models are remarkably similar to models unlearned using the full forget set in these dimensions.
% Additionally, we show the reliability of this coreset effect by comparing such coreset-unlearned models from various perspectives such as mode connectivity, emergent utility metrics and adversarial robustness against jailbreaking attacks. 
Finally, we uncover one possible downside of such coreset-unlearned models using finetuning based relearning attacks.
% We further validate RCE by showing that unlearned models using smaller forget sets are mode connected with unlearned models using the full forget set, demonstrate similar adversarial robustness and similar emergent utility capabilities. However, one difference between these models is demonstrated in relearning attacks in terms of relearning speed and robustness. 
Our results suggest unlearning in these benchmarks might be simpler than expected.

==> secs/coreset_main1.tex <==
\section{The ``Coreset"-like Effect in LLM Unlearning}
\label{sec: consistency}

In this section, we introduce the novel coreset-like effect through various data selection methods and demonstrate its \textbf{consistency} across the different LLM unlearning benchmarks. Specifically, we explore classic heuristic-based coreset selection techniques from the literature. Though these methods were primarily developed for learning, we adapt them to our unlearning process which we detail below.

\paragraph{\grand{}.} 
The main rationale behind this method \citep{paul2021deep} is that the importance of each sample $z_i$ from the forget set is captured by the expected gradient norm of the loss associated with that sample, where the expectation is taken over the unlearning trajectory. Thus the \grand{} score of $z_i$ is given by:
\begin{align}
\begin{array}{l}
  \chi(z_i) =  \mathbb E_{\btheta_t} \| \nabla_{\btheta_t} [\lf(z_i; \btheta_t) + \lambda \lr( z; \btheta_t) ] \|_2 \ ; \ \text{where} \  z \sim \Dr
\end{array}
\label{eq:grand}
\end{align}
Here $\lf$ and $\lr$ are specified in \eqref{eq: LLM_MU}, where $\lf$ changes according to the unlearning method as specified before. In our experiments, we consider the trajectory of unlearning for 10 epochs for the purpose of computing the above expectation.
% \SP{I will check if their theorems hold here. I will check and update the above later. But if anyone has time, kindly check.}

\paragraph{Moderate.}   

\paragraph{\mink{}.}
The \mink{} method \citep{shi2024detecting} was developed to ascertain whether a given text appears in the original pretraining dataset. We use this metric as a data selection method for unlearning under the notion that data points not encountered during training are less influential in the unlearning process. In fact, in  \citep{shi2024detecting}, the authors demonstrated that the \textsc{Min-K\%} metric can be used as an effective indicator for assessing removal of knowledge after unlearning. 

For a given datapoint $z$, we calculate the log-likelihood of each token and choose a set of top $40\% (\text{K} = 40)$ of tokens with lowest value, called $\text{Min-K\%}(z)$. Then the score for $z$ is calculated as:
\begin{align}
\begin{array}{l}
  \mink{}(z) = \frac{1}{|\text{Min-K\%}(z)|} \sum_{z_i \in \text{Min-K\%}(z)}{ \log p(z_i | z_1, ..., z_{i-1}; \btheta)}
\end{array}
\label{eq:grand}
\end{align}






After computing the above scores for each sample $z$ in $\Df$, we choose samples with the top $\mathrm{p}$ scores to obtain $\mathcal S_\mathrm{f}^\mathrm{p}$. Additionally, we perform \random{} selection as described in Section\,\ref{sec: problemstmnt}.

\begin{figure}[htb]
\centering
\begin{tabular}{cccc}
 \hspace*{-8mm}
 \includegraphics[width=.24\textwidth]{Figs/CLE_RMU_bio_Fig2.pdf}    &  
 \hspace*{-3.9mm}
 \includegraphics[width=.24\textwidth]{Figs/CLE_RMU_cyber_Fig2.pdf} &
 \hspace*{-3.9mm}
 \includegraphics[width=.24\textwidth]{Figs/CLE_NPO_bio_Fig2.pdf}    &  
 \hspace*{-3.9mm}
 \includegraphics[width=.24\textwidth]{Figs/CLE_NPO_cyber_Fig2.pdf} \\
{\footnotesize{(a) RMU, WMDP-Bio}}
& {\footnotesize{(b) RMU, WMDP-Cyber}}
& {\footnotesize{(a) NPO, WMDP-Bio}}   & {\footnotesize{(b) NPO, WMDP-Cyber}} 
\end{tabular}
\vspace*{-2mm}
\caption{\small{Unlearning Performance (UE) and Model Utility using MMLU (UT) remains surprisingly consistent with \random{} selection from the forget set in WMDP. The results are averaged over 5 random trials.
}}
  \label{fig: random_sufficient}
\end{figure}



% \noindent \textbf{Random Selection.}


% In this section, we provide various insights from our experiments on WMDP and MUSE which elucidate the coreset-like phenomenon. 

\subsection{Surprising Sufficiency of Random Selection.} As elucidated in Section\, \ref{sec: problemstmnt} and \reffig{fig: coreset-motivation}, we found that a randomly selected subset from the forget set was sufficient for performing unlearning in WMDP-Bio using RMU. To further investigate this phenomenon, we choose more random subsets from WMDP using 5 different seeds and perform unlearning using RMU and NPO. Surprisingly, we find that surprisingly, the ``coreset''-like effect is still preserved using just random selection \thatis these subsets perform on par with the full original $\Df$. As shown in \reffig{fig: random_sufficient}, we find that for RMU, even 1\% of the forget set is sufficient for comparable unlearning performance while for NPO, 5\% of the forget set is sufficient for unlearning. Its noteworthy that it comes at \textbf{no cost} of model utility. 

WMDP primarily measures on \textit{knowledge} unlearning and contains QA pairs in a MCQ format. Thus its imperative to investigate this random ``coreset'' sufficiency condition for \textit{data} unlearning using a non-MCQ evaluation, which is done using the MUSE benchmark. 
For MUSE, random selection of 5\% and 10\% of $\Df$ can also perform at par with the full forget set as seen in \reftab{tab: muse}. In fact, we observe that for RMU on MUSE-Books, random selection can infact \textbf{improve utility} when compared to the full forget set.
Its noteworthy that for MUSE-News, \textit{verbatim memorization} for models unlearned using 10\% of $\Df$ is much higher compared to those unlearned using $\Df$. However, we consider this to be successful \textit{data unlearning} because its comparable to the retrain model. 

\subsection{Advantages of systematic selection methods}
\input{Tables/wmdp-bio}
% \input{Tables/wmdp-cyber}
\input{Tables/musebooks}
% \input{Tables/musenews}

%%% We can put WMDP results side by side
\iffalse
\begin{figure}[h]
\begin{minipage}[th]{\textwidth}
\begin{minipage}[t]{0.5\textwidth}
\input{Tables/wmdp-bio}
\end{minipage}
\hfill
\begin{minipage}[t]{0.5\textwidth}
\input{Tables/wmdp-cyber}
\end{minipage}
\end{minipage}
% \vspace*{-4mm}
\end{figure}
\fi

We observe that heuristics-based coreset selection methods adapted to unlearning can infact provide help unlearning performance. As observed in \reftab{tab: wmdp-bio}, \SP{how do we say this? Need Mink and News results}








\subsection{Explaining random selection sufficiency: A keyword perspective}

To investigate the effect of the 




==> secs/outline.tex <==
\begin{center}
    \textbf{Outline of the paper}
\end{center}

\begin{enumerate}
\item{\textbf{Introduction}}
\begin{enumerate}
    \item What is MU and why is it important ? 
    \item Low data regime is an important area in MU due to various reasons:
    \begin{itemize}
        \item From a privacy perspective, when someone wants to unlearn some private data from a model, we cannot have a lot of data to perform that unlearning.
        \item In a practical scenario where we want to unlearn harmful knowledge, we may not have a lot of papers like WMDP - for example, on cutting-edge CBRN information. 
        \item A similar motivation for concept unlearning - search relevant literature.
    \end{itemize}
    \item Contributions List:
    \begin{enumerate}
        \item We establish a novel `Coreset Effect' in current LLM Unlearning benchmarks through extensive experiments in WMDP and MUSE using different unlearning methods such as NPO and RMU.
        \item We establish this effect for various heuristics-based coreset selection methods as well as random selection from the forget set.
        \item We explain the sufficiency of random selection of forget set using a keyword perspective.
        \item We demonstrate that models unlearned using random coresets are similar to models unlearned using the full forget set from various perspectives such as mode connectivity, adversarial robustness and emergent utilities.
        \item Finally, we uncover one potential disadvantage of such coreset-unlearned models using relearning attacks.
    \end{enumerate}
\end{enumerate}


\item{\textbf{Related Work}} 

\begin{enumerate*}
    \item LLM unlearning
    \item Coreset selection/dataset pruning for discriminative and generative models
    \item LLM unlearning data selection: recent coreset paper
    % \item 
\end{enumerate*}
% LLM unlearning; Coreset selection/dataset pruning for discriminative and generative models; Data selection for LLM unlearning,
% Mention about recent Coreset paper. 
% Mention Concept Unlearning papers. However, none of these papers are close to what we depict.

% \subsection{Sec: \SL{[Missing Problem Statement]}}

% \SL{Consider to add a motivating example using random data selection.}


\item{\textbf{Preliminaries and Problem Statement}}
 \begin{enumerate}
     \item Preliminaries on LLM unlearning : Only include generic unlearning equation.
     \item Provide \textbf{Figure} : Initial motivating experiment and the standard setting of WMDP-Bio and RMU: when we increase the number of epochs, we find that quite surprisingly, that even 1\% is successful. 
     \item Problem Statement: 
     \textit{Can we achieve comparable LLM unlearning performance in an extreme low-data regime across different benchmarks and methods ? Are such unlearned models similar to models unlearned with the full forget set ?}
     \item Experimental Setup: 
     \begin{itemize}
         \item We consider two prevalent LLM unlearning methods from two broad categories:
         \begin{itemize}
             \item PO based : NPO (describe briefly)
             \item Representation Based : RMU (describe briefly)
         \end{itemize}
         \item For WMDP, we consider the standard settings of RMU and each paper represents each datapoint.
         \item For MUSE, we consider each datapoint to be non-overlapping 2047 tokens from the full dataset.
         \item Provide reasons for not using TOFU
     \end{itemize}
 \end{enumerate}

\item{\textbf{Coreset Effects in LLM Unlearning}}

Here we provide brief preliminaries and describe our setup for the following methods: GraND, EL2N, Moderate, Random Selection.  We describe these using equations from Section 3.4.

\begin{enumerate}
\item{\textbf{Surprising Sufficiency of Random
Selection}}
Here we discuss the full-stack results for WMDP and MUSE using NPO and RMU.

\item{\textbf{Heuristic-Based Coreset Selection}}
Here we discuss the full-stack results for different coreset selection methods.

\item{\textbf{Explaining random selection sufficiency: A keyword perspective}}

\begin{enumerate}
    \item Include \textbf{Figure} showing:
    \begin{itemize}
        \item example question from evaluation set and unlearned models unlearning 'key' tokens.
        \item Histogram showing the frequency of such occurrence in the forget set
    \end{itemize} 
    \item Use the above as a hook to motivate finding such keywords from the forget set. 
    \item Methods:
    \begin{itemize}
        \item Include the prompt to LLM for finding keywords
        \item Method of unlearning using keywords
    \end{itemize}
    \item \textbf{Figure}: Overlapping keywords and explain how this is consistent with our previous observations.
    \item \textbf{Figure}: Unlearning performance for unlearning using keywords vs forget set. We conclude that keywords indeed have significant contribution in the unlearning performance.
\end{enumerate}
\end{enumerate}

\item{\textbf{Faithful Quality of Random Coreset-Unlearned Models}}


Here, we show how random coreset-unlearned models are indeed sufficient for unlearning from different perspectives.

\paragraph{Mode Connectivity.} We introduce mode connectivity, method and include \textbf{Figure}.

\paragraph{Emergent Utilities.}  We describe the emergent utility capabilities and include \textbf{Figure}. Demonstrate coreset Unlearned models may be beneficial in certain cases.

\paragraph{Adversarial robustness against input-level jailbreaking.} Describe enhanced GCG and include \textbf{Table}. 



\paragraph{A Possible Downside: Robustness to relearning attacks.} Describe relearning attacks and include \textbf{Figures}.

\item{\textbf{Conclusion and Future Work}}

\end{enumerate}


\iffalse 
\section{Sijia's Outline}
\begin{enumerate}
    \item Introduction
    \item Related Work
    \item Preliminaries and Problem Statement: 1) Preliminaries on LLM unlearning, 2) Motivating example on random forget data selection in WMDP for unlearning, 3) Proposed problem of our interest, 4)  Key Experiment Setups: Like IRM paper in Sec.2 \url{https://arxiv.org/pdf/2303.02343}
    \item (Method 1) \textbf{Coreset Effects} in LLM Unlearning: Surprising Sufficiency of Random Selection. 
    \begin{enumerate}
  %  \item Key Experiment Setups: Like IRM paper in Sec.2 \url{https://arxiv.org/pdf/2303.02343}
        \item RCE is consistent across unlearning methods \textbf{only if training ``properly''}
        \item RCE vs. Heuristics-based Coreset Selection Methods
        \item Coreset Effects in knowledge unlearning (WMDP/MUSE) vs. data unlearning (MUSE)
        \item Understanding the selected forget data from keyword importance
    \end{enumerate}
    \item (Method 2) \textbf{Faithful `Quality' of Coreset-Unlearned Models}
    \begin{enumerate}
        \item Model connectivity: Method and results
        % \item Other exploration of models' similarity
        \item Adversarial robustness against input-level jailbreaking 
        \item Emergent Utilities
        \item A Possible Downside: Robustness to white-based relearning attacks
    \end{enumerate}
    \item Conclusion and Future Work
\end{enumerate}
\fi 



==> secs/problemstatement.tex <==
\section{Preliminaries and Problem Statement}
\label{sec: problemstmnt}
In this section, we introduce the basics and methods LLM unlearning and provide an overview of our problem setup. 

\noindent \textbf{LLM Unlearning.}
In the general setup of LLM unlearning, we assume access to a forget set $\Df$ which contains the knowledge or data to be unlearned and a retain set $\Dr$ which usually does not contain any unlearning data. 
The goal of unlearning can then be achieved through solving the following optimization:
\begin{align}
\begin{array}{l}
 \displaystyle \min_{\boldsymbol{\theta}}
 \,\, {\mathbb E_{(x, \yf) \in \Df} [ \lf(\yf | x; \boldsymbol{\theta}) ]} + 
 \lambda { \mathbb E_{(x, y) \in \Dr} [ \lr( y | x; \boldsymbol{\theta}) ] }
\end{array}
\label{eq: LLM_MU}
\end{align} 
Here, $\lf$ and $\lr$ refers to the forget loss and retain loss respectively, which can take various forms as we will explain below. Usually, we perform unlearning on an initial LLM, which we call the reference model. We note that goal can either be unlearning memorized text from $\Df$ (unlearning verbatim memorization) or unlearning that knowledge present in $\Df$ (unlearning knowledge memorization) or both.
% Maybe Improve a bit here


We describe two popular methods of unlearning derived from two different principles, i.e. Preference Optimization (PO) based and Representation Misalignment based. From the PO angle, we consider \textbf{Negative Preference Optimization} \citep{zhang2024negative} which is shown to be the best among various PO methods. NPO treats $\Df$ as negative responses in preference optimization, while removing the positive response term. This results in the following loss which has been shown to obtain lower divergence rates when compared to various other unlearning approaches :
\begin{align}
  & \ell_{\mathrm{NPO}}(\boldsymbol{\theta}) =  \mathbb E_{(x,y) \in \Df} \underbrace{\left [    - \frac{2}{\beta} \log \sigma  \left ( - \beta \log \left ( \frac{\pi_{\btheta} (y | x) }{\pi_{\mathrm{ref}} (y | x)}\right ) \right ) 
    \right ]}_{\lf \  \text{specified in}  \ \eqref{eq: LLM_MU}}
\label{eq:NPO}
\end{align}
where $\sigma (t) = 1/(1+e^{-t})$ is the sigmoid function, $\beta > 0 $ is a hyperparameter. Minimizing the above forget loss drives output distribution of $\pi_{\btheta}$ \textit{i.e.} the model to be unlearned \textit{away} from the reference model $\pi_{\mathrm{ref}}$ for the samples from the forget set. In NPO, the retain loss $\lr$ is simply the prediction loss \textit{i.e.} the cross entropy loss between $x$ and $y$, which are obtained from $\Dr$.

From the Representation Misalignment angle, we consider \textbf{Representation Misdirection Unlearning} \citep{li2024wmdp} which aims to degrade the representation of the unlearned model for the forget set. This degradation is mainly done by making the hidden state activations of the unlearned model at some layer $l$ to be similar to a random unit vector $\mathrm{u}$, where each value is independently and uniformly sampled from $[0,1)$.
Unlike NPO, the retain loss here enforces alignment of the unlearned model representation with that of the reference model for the retain dataset. This is obtained in the following way:
\begin{align}
  & \ell_{\mathrm{RMU}}(\boldsymbol{\theta}) =  
  \mathbb E_{z_f \in \Df} \underbrace{\left [ \frac{1}{\mathrm{L_f}}\sum_{\text{token} \ t\in z_f} \|  \pi_{\btheta} (t) - c \cdot \mathrm{u}\|_2^2
    \right ]}_{\lf \  \text{specified in}  \ \eqref{eq: LLM_MU}} + \lambda
  \mathbb E_{z_r \in \Dr} \underbrace{\left [ \frac{1}{\mathrm{L_r}}\sum_{\text{token} \ t\in z_r} \|  \pi_{\btheta} (t) -\pi_{\mathrm{ref}} (t)\|_2^2
    \right ]}_{\lr \  \text{specified in}  \ \eqref{eq: LLM_MU}}
\label{eq:RMU}
\end{align}
where $\mathrm{L_f}$, $\mathrm{L_r}$ are the number of tokens in $z_f$, $z_r$ respectively and the hyperparameter $c$ is a hyperparameter. 





\noindent \textbf{LLM Unlearning benchmarks.}

WMDP, MUSE, why not tofu, others, Mention verbatim vs knolwedge metrics for MUSE, briefly explain UE, MMLU here.

\noindent \textbf{Experiment Setup and Motivation.} As mentioned in  Section\,\ref{sec: intro}, we want to explore unlearning in a low data regime. To achieve this using current benchmarks, we consider subsets of data from the full forget set $\Df = \{z_i\}_{i=1}^N$. Precisely, we choose a subset 
$\mathcal S_\mathrm{f}^\mathrm{p} \subset \Df , \  \text{s.t.} \  |\mathcal S_\mathrm{f}^\mathrm{p}| = \mathrm{pN}$, where $\mathrm{p}$ denotes the fraction of the total forget set. Hence, if we want to achieve unlearning with just 1\% of forget data, we need to choose $\mathcal S_\mathrm{f}^\mathrm{0.1} \subset \Df , \  \text{s.t.} \  |\mathcal S_\mathrm{f}^\mathrm{0.1}| = \mathrm{0.1N}$.
Thus, for WMDP, we consider the $z_i$ to be the  $i$-th paper and select a subset of these papers for exploring unlearning in a low data regime. Similarly, for MUSE, we divide the dataset into non-overlapping sets of 2047 consecutive tokens and $z_i$ comprises of each such set. 

\input{Fig_texs/fig1}

As an initial exploration, we perform unlearning using RMU on WMDP-Bio by taking simply taking random subsets of $\Df$ \textit{i.e.} $\mathcal S_\mathrm{f}^\mathrm{p} = \{z_\mathrm{f}^\mathrm{p}\}_{i=1}^{p\mathrm{N}}, \text{where} \  z_\mathrm{f,i}^\mathrm{p} \sim \mathcal{U}(\Df)$. By the standard settings of unlearning using RMU (which performs unlearning for a single epoch), we find that unlearning is unsuccessful when a low percentage of data from the forget set if chosen (for \eg when $p=0.1$). However, since the chosen dataset here is much smaller than the original full forget set, the total number of optimization steps for unlearning is quite less and as a result, we increase the number of epochs for which unlearning is performed. As shown in \textbf{Fig.\,\ref{fig: fig1}}, we encounter the surprising result that for $\Sf$, as we increase number of epochs, not only does the unlearning performance get better but it reaches the same performance when we unlearn using $\Df$, even when $p=0.01$. This also \textit{does not} come at a cost of utility. This inspires us to explore the following questions:
\begin{center}
	\setlength\fboxrule{0.0pt}
	\noindent\fcolorbox{black}[rgb]{0.95,0.95,0.95}{\begin{minipage}{0.98\columnwidth}
				{\bf (Consistency)}  Can we achieve comparable LLM unlearning performance in an extreme low-data regime (by taking small subsets of the original full forget set) consistently? \\
                {\bf (Faithfulness)} Are the subset-unlearned models similar to models unlearned with the full forget set ?
	\end{minipage}}
\end{center}



% \noindent \textbf{Motivating Example.} 





